Scalable Flow Simulations with the Lattice Boltzmann Method

The primary goal of the EuroHPC JU project SCALABLE is to develop an industrial Lattice Boltzmann Method (LBM)-based computational fluid dynamics (CFD) solver capable of exploiting current and future extreme scale architectures, expanding current capabilities of existing industrial LBM solvers by at least two orders of magnitude in terms of processor cores and lattice cells, while preserving its accessibility from both the end-user and software developer's point of view. This is accomplished by transferring technology and knowledge between an academic code (waLBerla) and an industrial code (LaBS). This paper briefly introduces the characteristics and main features of both software packages involved in the process. We also highlight some of the performance achievements in scales of up to tens of thousand of cores presented on one academic and one industrial benchmark case.

==> makefile <==
include document.mk
TEMPORARY_DIR=tmp
RELEASE_BUILD_DIR=${TEMPORARY_DIR}/release
DEBUG_BUILD_DIR=${TEMPORARY_DIR}/debug
VERBOSE_BUILD_DIR=${TEMPORARY_DIR}/verbose


ifndef VERBOSE
.SILENT:
endif

release:	${MAINFILE}.tex
	echo "Rendering ${MAINFILE}..."
	latexmk -bibtex -pdf -interaction=nonstopmode \
		-logfilewarnings- -quiet \
		-outdir=${RELEASE_BUILD_DIR} -gg -cd \
		-auxdir=${RELEASE_BUILD_DIR} \
		${MAINFILE}.tex 2> /dev/null
	cp ${RELEASE_BUILD_DIR}/${MAINFILE}.pdf ${MAINFILE}.pdf
	echo "${MAINFILE} rendered successfully."

debug:	${MAINFILE}.tex
	echo "Rendering ${MAINFILE}..."
	latexmk -bibtex -pdf -interaction=nonstopmode \
		-logfilewarnings- -quiet -shell-escape \
		-outdir=${DEBUG_BUILD_DIR} -gg -cd \
		-auxdir=${DEBUG_BUILD_DIR} \
		${MAINFILE}.tex
	cp ${DEBUG_BUILD_DIR}/${MAINFILE}.pdf ${MAINFILE}.pdf
	echo "${MAINFILE} rendered successfully."

verbose:	${MAINFILE}.tex
	echo "Rendering ${MAINFILE}..."
	latexmk -bibtex -pdf -interaction=nonstopmode \
		-logfilewarnings- -shell-escape -verbose \
		-outdir=${VERBOSE_BUILD_DIR} -gg -cd \
		-auxdir=${VERBOSE_BUILD_DIR} \
		${MAINFILE}.tex
	cp ${VERBOSE_BUILD_DIR}/${MAINFILE}.pdf ${MAINFILE}.pdf
	echo "${MAINFILE} rendered successfully."


clean:
	rm ${MAINFILE}.pdf


